Reconstructing Cell Lineage Trees from Phenotypic Features with Metric Learning

How a single fertilized cell gives rise to a complex array of specialized cell types in development is a central question in biology. The cells grow, divide, and acquire differentiated characteristics through poorly understood molecular processes. A key approach to studying developmental processes is to infer the tree graph of cell lineage division and differentiation histories, providing an analytical framework for dissecting individual cells' molecular decisions during replication and differentiation. Although genetically engineered lineage-tracing methods have advanced the field, they are either infeasible or ethically constrained in many organisms. In contrast, modern single-cell technologies can measure high-content molecular profiles (e.g., transcriptomes) in a wide range of biological systems. Here, we introduce CellTreeQM, a novel deep learning method based on transformer architectures that learns an embedding space with geometric properties optimized for tree-graph inference. By formulating lineage reconstruction as a tree-metric learning problem, we have systematically explored supervised, weakly supervised, and unsupervised training settings and present a Lineage Reconstruction Benchmark to facilitate comprehensive evaluation of our learning method. We benchmarked the method on (1) synthetic data modeled via Brownian motion with independent noise and spurious signals and (2) lineage-resolved single-cell RNA sequencing datasets. Experimental results show that CellTreeQM recovers lineage structures with minimal supervision and limited data, offering a scalable framework for uncovering cell lineage relationships in challenging animal models. To our knowledge, this is the first method to cast cell lineage inference explicitly as a metric learning task, paving the way for future computational models aimed at uncovering the molecular dynamics of cell lineage.

==> table/tbl-methods.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[ht]
\begin{tabular}{@{}llll@{}}
\toprule
Type of Linage Construction               & Idea                                                                                                                                                            & Approahces                                                                                                                                                             & Limitations                                                                                                                                                                                                                                                  \\ \midrule
Differentiation Trajectory Reconstruction & Cells with similar expression profiles arise from the same lineage and that cells with more similiarity between their expression  profiles are closely related. & \begin{tabular}[c]{@{}l@{}}Dimensionality reduction based algorithms;\\ Nearest neighbor graph-based algorithms;\\ RNA velocity based algorithms.\end{tabular}         & \begin{tabular}[c]{@{}l@{}}Relies on sufficient sampling of cells that transition between the different states in the lineage trajectory.\\ Phynotypic do not necessarily reflect the genetic relations between the true lineages of the cells.\end{tabular} \\
Genetic Lineage Tracing: Prospective      & Introducing reporter transgenes to label single founder cells. All descendants inherit the transgenes.                                                          & CRISPR-Cas9 Genome Editing based linage tracing                                                                                                                        & \begin{tabular}[c]{@{}l@{}}Require the introduction of exogeneous matrial ino the cell. It can be impossible to implement in a completely wide-type setting.\\ The tracing can only start after the introduction of the genetic labels.\end{tabular}         \\
Genetic Lineage Tracing: Retrospective    & Make use of inheritable elements that accumulate over time.                                                                                                     & \begin{tabular}[c]{@{}l@{}}scDNA-seq and CNV\\ scGWS and SNV, indels, repeat regions.\\ scEpigenetic markers: DNA methylation and DNA hydroxymethylation.\end{tabular} & \begin{tabular}[c]{@{}l@{}}CNV is low in healthy somatic tissues;\\ scWGS and scWES are too sparse;\end{tabular}                                                                                                                                             \\ \bottomrule
\end{tabular}
\end{table}

==> table/tbl-partial_label_celegans_dev_full_wide.tex <==
\begin{table}[ht]
\centering
\scriptsize
\scalebox{0.65}{ 
\begin{tabular}{l|rrrrrr|rrrrrr|rrrrrr}
\hline
             & \multicolumn{6}{l|}{Known Fraction: 0.8}                                                                                                                                        & \multicolumn{6}{l|}{Known Fraction: 0.5}                                                                                                                                        & \multicolumn{6}{l}{Known Fraction: 0.3}                                                                                                                                        \\ \hline
Quartets     & \multicolumn{1}{l}{}         & \multicolumn{1}{l}{}      & \multicolumn{1}{c}{All}   & \multicolumn{1}{c}{Known}   & \multicolumn{1}{c}{Partial} & \multicolumn{1}{c|}{Unknown} & \multicolumn{1}{l}{}         & \multicolumn{1}{l}{}      & \multicolumn{1}{c}{All}   & \multicolumn{1}{c}{Known}   & \multicolumn{1}{c}{Parital} & \multicolumn{1}{c|}{Unknown} & \multicolumn{1}{l}{}         & \multicolumn{1}{l}{}      & \multicolumn{1}{c}{All}   & \multicolumn{1}{c}{Known}   & \multicolumn{1}{c}{Parital} & \multicolumn{1}{c}{Unknown} \\ \hline
\# Quartets  & \multicolumn{1}{l}{}         & \multicolumn{1}{l}{}      & 4,249,575                 & 1,663,740                   & 2,579,850                   & 5,985                        & \multicolumn{1}{l}{}         & \multicolumn{1}{l}{}      & 4,249,575                 & 249,900                     & 3,749,775                   & 249,900                      & \multicolumn{1}{l}{}         & \multicolumn{1}{l}{}      & 4,249,575                 & 27,405                      & 3,193,380                   & 1,028,790                   \\
\% Quartets  & \multicolumn{1}{l}{}         & \multicolumn{1}{l}{}      & 1                         & 0.3915                      & 0.6071                      & 0.0014                       & \multicolumn{1}{l}{}         & \multicolumn{1}{l}{}      & 1                         & 0.0588                      & 0.8824                      & 0.0588                       & \multicolumn{1}{l}{}         & \multicolumn{1}{l}{}      & 1                         & 0.0064                      & 0.7515                      & 0.2421                      \\ \hline
             & \multicolumn{1}{c}{Train RF} & \multicolumn{1}{c}{$\Delta$\%RF} & \multicolumn{1}{c}{$\Delta$\%QD} & \multicolumn{1}{c}{$\Delta$\%K-QD} & \multicolumn{1}{c}{$\Delta$\%P-QD} & \multicolumn{1}{c|}{$\Delta$\%U-QD} & \multicolumn{1}{c}{Train RF} & \multicolumn{1}{c}{$\Delta$\%RF} & \multicolumn{1}{c}{$\Delta$\%QD} & \multicolumn{1}{c}{$\Delta$\%K-QD} & \multicolumn{1}{c}{$\Delta$\%P-QD} & \multicolumn{1}{c|}{$\Delta$\%U-QD} & \multicolumn{1}{c}{Train RF} & \multicolumn{1}{c}{$\Delta$\%RF} & \multicolumn{1}{c}{$\Delta$\%QD} & \multicolumn{1}{c}{$\Delta$\%K-QD} & \multicolumn{1}{c}{$\Delta$\%P-QD} & \multicolumn{1}{c}{$\Delta$\%U-QD} \\ \hline
PhyloDist    & 0.0242                       & \textbf{0.4479}           & \textbf{0.8424}           & \textbf{0.9995}             & \textbf{0.7416}             & \textbf{0.4649}              & 0.0116                       & 0.0921                    & \textbf{0.6094}           & \textbf{0.9989}             & \textbf{0.5980}             & \textbf{0.3983}              & 0.0000                       & -0.0234                   & \textbf{0.3680}           & \textbf{1.0000}             & \textbf{0.4007}             & \textbf{0.2505}             \\
PhyloDist-G  & 0.0313                       & 0.4112                    & \textbf{0.8374}           & \textbf{0.9995}             & \textbf{0.6999}             & 0.3715                       & 0.0162                       & \textbf{0.0997}           & \textbf{0.6024}           & \textbf{0.9991}             & \textbf{0.5709}             & \textbf{0.3519}              & 0.0082                       & -0.0201                   & 0.3356                    & 0.9990                      & 0.3395                      & 0.1803                      \\
Triplet      & 0.4544                       & 0.1753                    & 0.7282                    & 0.8950                      & 0.6240                      & 0.3391                       & 0.3032                       & 0.0486                    & 0.5046                    & 0.8787                      & 0.4930                      & 0.3043                       & 0.1564                       & -0.0015                   & 0.3578                    & 0.8886                      & 0.3840                      & \textbf{0.2628}             \\
Triplet-G    & 0.4188                       & 0.2008                    & 0.7388                    & 0.8949                      & 0.6184                      & \textbf{0.3945}              & 0.3194                       & 0.0674                    & 0.5196                    & 0.8833                      & 0.4994                      & 0.3077                       & 0.1687                       & -0.0172                   & \textbf{0.3522}           & \textbf{0.8901}             & \textbf{0.3634}             & 0.2203                      \\
Quadruplet   & 0.0655                       & 0.4032                    & 0.7960                    & 0.9531                      & 0.6970                      & \textbf{0.4350}              & 0.0231                       & 0.1153                    & 0.5485                    & 0.9342                      & 0.5371                      & 0.3398                       & 0.0082                       & -0.0203                   & 0.3582                    & 0.9181                      & \textbf{0.3858}             & \textbf{0.2591}             \\
Quadruplet-G & 0.0598                       & \textbf{0.4115}           & 0.7843                    & 0.9364                      & 0.6625                      & 0.3199                       & 0.0394                       & \textbf{0.1027}           & 0.5397                    & 0.9416                      & 0.5145                      & 0.2993                       & 0.0288                       & -0.0161                   & \textbf{0.3638}           & 0.9401                      & 0.3618                      & 0.2084                      \\ \hline
\end{tabular}
}
\end{table}

==> tex/app_furture_supervised.tex <==
% There are some observations.
% \begin{itemize}
%     \item C.elegans-Dev: PhyloDist-Transformer achieves an RF distance of 0.246, significantly improving upon the raw data baseline (0.929) and demonstrating better performance than PhyloDist-FC (0.400). Permuting leaves, cells, or genes leads to substantial degradation in tree quality, confirming that the learned structure is meaningful and sensitive to input organization.
%     \item C.elegans-Packer: Although the dataset is more complex (295 leaves), PhyloDist-Transformer still outperforms the raw baseline by a large margin, yielding an RF distance of 0.571 compared to 0.955. This improvement illustrates PhyloDist’s ability to handle larger and more complex lineage trees.
%     \item Methylation Dataset: The PhyloDist-Transformer embedding again shows a clear advantage over the raw baseline (0.4328 vs. 0.71), indicating that our method can generalize to diverse data types, including epigenetic measurements.
% \end{itemize}


% \subsection{Strategies for Unsupervised Learning}
% In practical scenarios, neither the true order of quartet sums nor partial lineage constraints may be available. Under these fully unsupervised conditions, the model must rely solely on the intrinsic structure of the data. Here, we explore two complementary directions: introducing additional inductive biases in metric learning and leveraging adaptive quartet selection methods.

% \subsubsection{Metric Learning with a Learnable Linear Embedding}
% Our first approach is to enhance metric learning by introducing a learnable linear embedding matrix $G$. This embedding filters out irrelevant features and focuses the model on lineage-relevant signals. Formally, we modify the loss function as follows:
% \begin{equation}
% \min_f \mathcal{L} = \mathcal{L}_{\text{additivity}}(f, GX) + \Omega(f, G, X) 
% \end{equation}
% where
% \[
% \Omega(f, G, X) = \frac{1}{N} \| \mathcal{D}(f(GX)) - \mathcal{D}(X) \|_F^2 + \|G-I\|.
% \]

% By penalizing the deviation of  $G$ from the identity matrix $I$, we encourage $G$ to remain close to a simple transformation while selectively attenuating noise. In simulated datasets, this approach successfully filters out independent noise by setting some diagonal entries of  $G$ near zero, enabling the model to recover the correct tree structure without explicit prior constraints. However, this strategy has not yet succeeded in improving performance on the C. elegans datasets, indicating that more sophisticated approaches may be needed for complex biological data.

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.45\linewidth]{fig/simulation-1.png}
%     \includegraphics[width=0.45\linewidth]{fig/simulation-2.png}    
%     \caption{Unsupervised learning dynamics on simulated datasets with the learnable linear embedding $G$}
%     \label{fig:PhyloDist unsupervised learning dynamics on simulation datasets}
% \end{figure}

% \subsubsection{Quartet Mining for High-Confidence Constraints}
% Our second direction focuses on identifying quartets that can be assigned high-confidence topologies without prior knowledge. Given a quartet, there are three possible topologies. We can estimate the edge lengths for each topology via least squares (Section~\ref{preliminaries}) and compute the residual between the inferred additive distance matrix and the observed distances. An example is shown in \ref{fig:topology residual}. By comparing the residuals across the three candidate topologies, we define a confidence score for each topology:
% \[
% \text{confidence score(r1)} = \frac{1/r_1}{1/r_1 + 1/r_2 + 1/r_3}
% \]
% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.5\linewidth]{fig/residual.png}
%     \caption{Estimating residuals and confidence scores for quartet topologies.}
%     \label{fig:topology residual}
% \end{figure}

% Applying this procedure to the C. elegans-dev dataset, we sampled 40,960 quartets and estimated their topologies. Selecting all quartets yields a 0.45 accuracy in recovering the correct topology. Restricting to the top $0.1\%$ most confident quartets improves accuracy to 0.5894. While this is better, it remains insufficient for reliable unsupervised reconstruction. Additional constraints, such as ensuring that a chosen set of quartets are mutually compatible, may further improve the quality of these high-confidence inferences.

==> tex/app_identifiability.tex <==
\section{Tree Identifiability Theorem}
\begin{theorem}[Tree Identifiability for Brownian Motion with Multiple Traits]
\label{thm:BM-tree-identifiability}
Let $T$ be a rooted tree on $n$ leaves with strictly positive edge lengths, 
and let 
\[
   x^* \;:=\; \min_{e \in E(T)} \ell_e \;>\; 0
\]
denote the minimum edge length in $T$. 
Here, ``edge length'' $\ell_e$ can be viewed as the contribution to the \emph{expected} squared distance from edge $e$ (e.g., $\ell_e = \text{trace}(\Sigma_e)$ in a Gaussian increment model).

Suppose we observe $M$ i.i.d.\ \emph{Brownian replicates} of a continuous-state process on $T$, indexed by $m = 1, \dots, M$. Concretely, for each $m$:

\begin{enumerate}
  \item The random vector $X^m(v) \in \mathbb{R}^d$ (where $d \ge 1$) is assigned to each vertex $v \in T$.
  \item Each edge $e=(u \to v)$ carries an independent Gaussian increment $\Delta_e^m := X^m(v) - X^m(u)$ of mean $\mathbf{0}$ and covariance $\Sigma_e$.
  \item Across edges, increments $\Delta_e^m$ are mutually independent. 
  \item Across replicates, all processes are i.i.d.\ copies of the same Brownian model on $T$.
\end{enumerate}
For leaves $i,j$, define the \emph{empirical squared distance}
\[
  \widehat{D}_M(i,j)
  \;=\;
  \frac{1}{M} \,\sum_{m=1}^M \bigl\|X^m(i) - X^m(j)\bigr\|^2.
\]
Let $D(i,j) = \mathbb{E}[\|X^m(i) - X^m(j)\|^2]$ be the \emph{true} (theoretical) expected distance, which is known to be additive:
\[
   D(i,j) 
   \;=\; \sum_{e \in \mathrm{path}(i,j)} \text{trace}(\Sigma_e).
\]
Then for any $\epsilon > 0$, there exists an integer $M_0$ (depending on $\epsilon, n, d$ and the parameters $\{\Sigma_e\}$) such that, for all $M \ge M_0$, the following holds with probability at least $1 - \delta$ (where $\delta \to 0$ as $M \to \infty$):

\[
  \max_{1 \le i,j \le n}
      \bigl|\widehat{D}_M(i,j) \;-\; D(i,j)\bigr|
  \;\le\; \epsilon.
\]

In particular, if $\epsilon \le x^*/2$, then by Atteson's Theorem~\citep{atteson_performance_1999}, any distance-based method satisfying that theorem (e.g.\ Neighbor-Joining) will exactly recover the tree $T$ with high probability.
\end{theorem}

==> tex/app_key_challenges.tex <==
\section{Key Challenges}
Reconstructing a cell lineage tree from \emph{phenotypic} data is conceptually related to phylogenetics, where aligned DNA or protein sequences are used to infer evolutionary relationships. Methods in classical phylogenetics typically assume a well-defined stochastic model of sequence evolution (e.g., Jukes–Cantor) and estimate both topology and branch lengths of the tree under this model \citep{felsenstein_inferring_2003}. While these methods have proven empirically effective, the situation for transcriptome-based lineage reconstruction is far less established, for reasons outlined below.

\paragraph{Challenge 1: Unknown evolution model} The success of phylogenetic lineage reconstruction methods has largely relied on well-established stochastic models of genetic evolution, which often provide clear optimization objectives. However, little research has been conducted to identify an evolutionary model that accurately characterizes empirical transcriptome data. In fact, whether transcriptomic information alone is sufficient to reliably reconstruct evolutionary lineages remains an open question. Nonetheless, previous studies have explored the use of transcriptome data as auxiliary information for genetic lineage reconstruction. It has been demonstrated that heritable gene expression patterns can distinguish between symmetric and asymmetric cell fate decisions and have been leveraged to reconstruct portions of multicellular structures \citep{phillips_memory_2019,shaffer_memory_2020,ruckert_clonal_2022,mold_clonally_2024}. Moreover, selecting specific genes has been shown to enhance the clustering of cells that share lineage labels \citep{eisele_gene-expression_2024}. These findings suggest that reconstructing lineage solely from transcriptomic data is a promising direction.

\paragraph{Challenge 2: Non-causal and confounding features} Gene expression captures a cell’s functional and regulatory states, many of which may be transient, environmentally induced, or otherwise unrelated to the heritable lineage history. Factors such as cell cycle stage, nutrient availability, or niche-specific signaling can introduce large expression shifts that mask or distort the true ancestral relationships.

\paragraph{Challenge 3: Poor distance proxies} Many genes change their RNA counts in response to \emph{intrinsic} processes (\textit{e.g.}, cell cycle) or to \emph{extrinsic} factors (\textit{e.g.}, cell signaling, environmental conditions, or spatial position). The underlying lineage history information can be obscured by these factors. Moreover, distantly related cells may exhibit convergent expression profiles if they perform similar biological functions. Indeed, in \textit{C. elegans}, transcriptomic similarity initially correlates with lineage relationships but diverges after gastrulation once cells commit to specialized fates, illustrating how true lineage information might be lost in the broad transcriptome \citep{packer_lineage-resolved_2019,qiu_systematic_2022}.

\paragraph{Challenge 4: Inherent uncertainty in getting biological data}
Defining node representations is difficult. In phylogenetics, each taxon—be it a species of animal or a strain of virus—is typically well-defined and has a clear ontological status. Analogously, one might expect that the taxa in a cell lineage tree correspond to distinct cell types. In reality, cells rarely fall into sharply defined ``types.'' They often occupy a continuum of states, making it unclear how best to group cells into discrete lineage nodes. Moreover, the mainstream single-cell technology makes destructive measurements, such that we cannot continuously observe the molecular states of the same cell throughout its entire lineage; instead, we obtain snapshots of cells at various developmental stages. This sampling procedure further complex the grouping. \citep{kim_rna_2010}

\paragraph{Challenge 5: Scarcity of ground-truth lineage annotations}
Comprehensive and accurate lineage annotations are scarce. To solve the learning task and evaluate the performance. We need a ground-truth corpus with annotated lineages. The \emph{Caenorhabditis} species of nematode worms are uniquely suited among major model organisms because they show repeatable invariant cell lineage trees that have been already identified through direct observation. Pioneering work in the 1970s and 1980s by Sydney Brenner, John Sulston, and others meticulously documented the lineage of C. elegans using manual observations.\citep{sulston_embryonic_1983}. However, such well characterized cell lineage tree for a whole organism is unique to this group of organisms. In limited cases, some degree of ground-truth cell lineage annotations might be available in other organisms, but such supervised data is extremely limited  \citep{domcke_reference_2023}. 

Given these challenges, our goal is not to devise a more intricate transcriptomic evolution model but rather to embed high-dimensional phenotypic profiles into a \emph{metric space} whose distance function captures genuine lineage relationships. As we demonstrate, applying metric learning to transcriptomic data can overcome the above challenges by isolating heritable signals from confounding factors, thus enabling effective tree reconstruction without explicit assumptions about the transcriptome’s evolutionary dynamics.

==> tex/evaluations.tex <==



==> tex/pf_high_level_partition.tex <==
\subsection{Fraction of Unknown Quartets on Full Balanced Binary Tree}\label{appendix:fraction_of_unkown_quartet_full_binary_tree}
Suppose we have a full binary tree with $N$ leaves. Suppose we know the topology down to level $L$. So there are $k = 2^L$ clades at level L. Each clade has $n = \frac{N}{2^L}$ leaves. 
The number of all the quartets is
\[
Q = \binom{n}{4} \approx \frac{N^4}{24}.
\]

When $L=1$, the fraction of known quartets is
\[
Q_{1}= \frac{\binom{n/2}{2} \binom{n/2}{2}}{\binom{n}{4}} = 
\frac{3\,n(n-2)}{8\,(n-1)(n-3)}
\;\approx\; \frac{3n^2}{8n^2}
\;=\; \frac{3}{8}
\;=\; 0.375
\]
So the fraction of unknown quartet $Q_0 = 1 - Q_1 = 0.625$.

When $L >1$, the number of unknown quartets is:
\begin{align*}
Q_0 =& \underbrace{\sum_{i=1}^{k} \binom{n}{4}}_{\text{(4)-type}}
\;+\;
\underbrace{\sum_{i=1}^{k} \binom{n}{3}\,(N - n)}_{\text{(3+1)-type}}\\
\;=&\;
k \,\binom{n}{4}
\;+\;
k \,\binom{n}{3}\,(N-n) \\
\;\approx\;&
2^L \times \frac{n^4}{24}
\;+\;
2^L \times \frac{n^3}{6}\,\bigl(N\bigr).
\end{align*}

\[
2^L \times \frac{n^4}{24}
\;=\;
2^L \times \frac{\bigl(N/2^L\bigr)^4}{24}
\;=\;
\frac{N^4}{24}\,\frac{2^L}{(2^L)^4}
\;=\;
\frac{N^4}{24}\,\frac{1}{2^{3L}}.
\]

\[
2^L \times \frac{n^3}{6}\,N
\;=\;
2^L \times \frac{\bigl(N/2^L\bigr)^3}{6}\,N
\;=\;
\frac{N^4}{6}\,\frac{2^L}{(2^L)^3}
\;=\;
\frac{N^4}{6}\,\frac{1}{2^{2L}}.
\]

Therefore, the fraction of unknown quartets is roughly
\[Q_{0}=
\frac{\frac{N^4}{24}\,\frac{1}{2^{3L}} \;+\; \frac{4\,N^4}{24}\,\frac{1}{2^{2L}}}{\frac{N^4}{24}}
\;=\;
\frac{1}{2^{3L}}
\;+\;
\frac{4}{2^{2L}}
\;=\;
\frac{1}{2^{3L}}
\;+\;
\frac{1}{2^{2L-2}}.
\]

Therefore, the fraction of unknown quartets is independent to the size of the tree. 

\begin{itemize}
    \item $L=1$, $Q_{0}=0.625$.
    \item $L=2$, $Q_{0}=0.265$.
    \item $L=3$, $Q_{0}=0.064$.
\end{itemize}

